Quantum Machine Learning using the ZXW-Calculus

The field of quantum machine learning (QML) explores how quantum computers can be used to more efficiently solve machine learning problems. As an application of hybrid quantum-classical algorithms, it promises a potential quantum advantages in the near term. In this thesis, we use the ZXW-calculus to diagrammatically analyse two key problems that QML applications face. First, we discuss algorithms to compute gradients on quantum hardware that are needed to perform gradient-based optimisation for QML. Concretely, we give new diagrammatic proofs of the common 2- and 4-term parameter shift rules used in the literature. Additionally, we derive a novel, generalised parameter shift rule with 2n terms that is applicable to gates that can be represented with n parametrised spiders in the ZXW-calculus. Furthermore, to the best of our knowledge, we give the first proof of a conjecture by Anselmetti et al. by proving a no-go theorem ruling out more efficient alternatives to the 4-term shift rule. Secondly, we analyse the gradient landscape of quantum ans\"atze for barren plateaus using both empirical and analytical techniques. Concretely, we develop a tool that automatically calculates the variance of gradients and use it to detect likely barren plateaus in commonly used quantum ans\"atze. Furthermore, we formally prove the existence or absence of barren plateaus for a selection of ans\"atze using diagrammatic techniques from the ZXW-calculus.

==> header/environments.tex <==
\newlength{\blockindent}
\setlength{\blockindent}{8mm}

\newtheorem{lemma}{Lemma}[chapter]
\newtheorem{proposition}[lemma]{Proposition}
\newtheorem{fact}[lemma]{Fact}
\newtheorem{theorem}[lemma]{Theorem} %Uncomment this line if you want to use usual theorems from ntheorem
\newtheorem{corollary}[lemma]{Corollary}
\newtheorem{definition}[lemma]{Definition}
\newtheorem{exercise}[lemma]{Exercise}
\newtheorem{example}[lemma]{Example}
\newtheorem{remark}[lemma]{Remark}
\newtheorem{assumption}[lemma]{Assumption}

%% Beweise
\theoremstyle{nonumberplain}
\theorembodyfont{\normalfont}
\theoremsymbol{\qed}
\newtheorem{proof}{Proof}
\theoremclass{LaTeX}

%% Boxed prooftree: https://tex.stackexchange.com/questions/214012/latex-bussproofs-package-prooftrees-on-same-line
\newenvironment{bprooftree}{\leavevmode\hbox\bgroup}{\DisplayProof\egroup}



==> header/header.tex <==
\makeatletter

% Packages needed
\usepackage[utf8]{inputenc}
\usepackage{geometry}
%\usepackage[small,compact]{titlesec}
%\usepackage[compact]{titlesec}
\usepackage{titlesec}
\usepackage[final]{listings}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{tipa}
\usepackage[english]{babel}
\usepackage{lstautogobble}
\usepackage{xparse}
\usepackage{needspace}
\usepackage{xspace}
\usepackage{mathpartir}
\usepackage{tikz}
\usetikzlibrary{arrows}
\usetikzlibrary{fit}
\usetikzlibrary{positioning}
%\usepackage[amsmath,hyperref,thmmarks]{ntheorem}
\usepackage{amsthm}
\usepackage{parskip}
\usepackage{scrextend}
\usepackage{wrapfig}
\usepackage[nottoc]{tocbibind}
\usepackage{caption}
\usepackage{aligned-overset}
\usepackage[createShortEnv]{proof-at-the-end}

\usepackage{tikzit}
\input{quantum.tikzdefs}
\input{quantum.tikzstyles}


% Ignore 'draft' flag for hyperref
\hypersetup{final}



% For the font
%\usepackage[T1]{fontenc}
%\usepackage{tgpagella}
%\usepackage{newpxmath}
%%\usepackage[euler-digits,small]{eulervm}
%\linespread{1.025}              % Palatino leads a little more leading

\usepackage{fancyhdr}
\usepackage[obeyDraft]{todonotes}
\setlength{\marginparwidth}{3cm}

\usepackage[toc]{glossaries}
\usepackage{natbib}
\bibpunct{[}{]}{,}{n}{,}{;}

%\usepackage[breaklinks, draft=false, pdfusetitle]{hyperref}


% Double spacing
\usepackage[nodisplayskipstretch]{setspace}

% Don't use double spacing in displaymath: https://tex.stackexchange.com/questions/324091/single-spaced-equations-in-double-spaced-documents
\usepackage{etoolbox}
\setdisplayskipstretch{}
\makeatletter
\newcommand*\MySingleSpacePatch{%
	\begin{singlespace}%
		\vskip -\baselineskip
		\noindent
		\dimen@ \hsize
		\advance \dimen@ \p@
		\hskip \dimen@ \@minus \tw@\p@ % 2pt and not 1pt because I am paranoid
		\null
	}
	\newcommand*\EndMySingleSpacePatch{%
	\end{singlespace}%
	\noindent\ignorespaces
}
\makeatother
\BeforeBeginEnvironment{equation*}{\MySingleSpacePatch}
\AfterEndEnvironment{equation*}{\EndMySingleSpacePatch}
\BeforeBeginEnvironment{gather*}{\MySingleSpacePatch}
\AfterEndEnvironment{gather*}{\EndMySingleSpacePatch}
\BeforeBeginEnvironment{align*}{\MySingleSpacePatch}
\AfterEndEnvironment{align*}{\EndMySingleSpacePatch}
\BeforeBeginEnvironment{equation}{\MySingleSpacePatch}
\AfterEndEnvironment{equation}{\EndMySingleSpacePatch}
\BeforeBeginEnvironment{gather}{\MySingleSpacePatch}
\AfterEndEnvironment{gather}{\EndMySingleSpacePatch}
\BeforeBeginEnvironment{align}{\MySingleSpacePatch}
\AfterEndEnvironment{align}{\EndMySingleSpacePatch}


% My packages
\usepackage{bm}
\usepackage{multicol}
\usepackage{stmaryrd}
\usepackage{csquotes}
\usetikzlibrary{arrows.meta,tikzmark,calc}
\usepackage{bussproofs}
\usepackage{mathtools}
%\usepackage{mathrsfs} %\mathscr{}
\usepackage{cleveref}
\usepackage{graphicx,nicefrac}
\usepackage{changepage}
\usepackage{pgf}
\usepackage{pgfplots}
\usepackage{float}

%\titlespacing*{\section} {0pt}{3.5ex plus 1ex minus .2ex}{2.3ex plus .2ex}
%\titlespacing*{\subsection} {0pt}{3.25ex plus 1ex minus .2ex}{1.5ex plus .2ex}


%% Geometrie
\newdimen\lines

\newlength{\exb}
\settowidth{\exb}{\normalfont x}
\geometry{%
  a4paper,%
  includehead,% (=> head is part of total body)
  includefoot,% (=> foot is not part of total body)
  hmargin=3.5cm,
  vmargin=3cm,
  headheight=1\lines,%
  headsep=0.5cm,%
  %foot=4\lines,% (bottom of text body |---| _bottom_ of foot)
  hcentering%
}%



%\newlength{\blockindent}
%\setlength{\blockindent}{8mm}

\newtheorem{lemma}{Lemma}[chapter]
\newtheorem{proposition}[lemma]{Proposition}
\newtheorem{fact}[lemma]{Fact}
\newtheorem{theorem}[lemma]{Theorem} %Uncomment this line if you want to use usual theorems from ntheorem
\newtheorem{corollary}[lemma]{Corollary}
\newtheorem{definition}[lemma]{Definition}
\newtheorem{exercise}[lemma]{Exercise}
\newtheorem{example}[lemma]{Example}
\newtheorem{remark}[lemma]{Remark}
\newtheorem{assumption}[lemma]{Assumption}
\newtheorem{hypothesis}[lemma]{Hypothesis}

% Theorem title in bold
\makeatletter
\def\th@plain{%
	\thm@notefont{}% same as heading font
	\itshape % body font
}
\def\th@definition{%
	\thm@notefont{}% same as heading font
	\normalfont % body font
}
\makeatother

% "Proof." in bold:
\makeatletter
\renewenvironment{proof}[1][\proofname] {\par\pushQED{\qed}\normalfont\topsep6\p@\@plus6\p@\relax\trivlist\item[\hskip\labelsep\bfseries#1\@addpunct{.}]\ignorespaces}{\popQED\endtrivlist\@endpefalse}
\makeatother


% Set text for proof-at-end package
\pratendSetGlobal{text link={\textbf{Proof.} See \Cref{chap:appendix-proofs}. \hfill\hyperref[proof:prAtEnd\pratendcountercurrent]{$\downarrow$}}}


%\theoremstyle{nonumberplain}
%\theorembodyfont{\normalfont}
%\theoremsymbol{\ensuremath\square}
%\newtheorem{proof}{Proof.}
%\theoremclass{LaTeX}





\allowdisplaybreaks

\makeatother



% Macros

%Axioms
\newcommand{\bOne}{\hyperref[eqn:b1]{\bm{\mathit{b_1}}}}
\newcommand{\bTwo}{\hyperref[eqn:b2]{\bm{\mathit{b_2}}}}
\newcommand{\bThree}{\hyperref[eqn:b3]{\bm{\mathit{b_3}}}}
\newcommand{\ety}{\hyperref[eqn:ety]{\bm{\mathit{ety}}}}
\newcommand{\eu}{\hyperref[eqn:eu]{\bm{\mathit{eu}}}}
\newcommand{\triTipZero}{\hyperref[eqn:tri1]{\bm{\mathit{tri_1}}}}
\newcommand{\triTipOne}{\hyperref[eqn:tri2]{\bm{\mathit{tri_2}}}}
\newcommand{\zero}{\hyperref[eqn:zero]{\bm{\mathit{zero}}}}
\renewcommand{\sf}{\hyperref[eqn:sf]{\bm{\mathit{sf}}}}
\newcommand{\cc}{\hyperref[eqn:cc]{\bm{\mathit{cc}}}}
\renewcommand{\sc}{\hyperref[eqn:sc]{\bm{\mathit{sc}}}}
\newcommand{\hh}{\hyperref[eqn:hh]{\bm{\mathit{hh}}}}
\newcommand{\cp}{\hyperref[eqn:cp]{\bm{\mathit{cp}}}}
\newcommand{\p}{\hyperref[eqn:pi]{\bm{\pi}}}
\newcommand{\id}{\hyperref[eqn:id]{\bm{\mathit{id}}}}
\newcommand{\ho}{\hyperref[eqn:hopf]{\bm{\mathit{ho}}}}  % Hopf
\newcommand{\wdc}{\hyperref[eqn:wdc]{\bm{\mathit{wdc}}}}
\newcommand{\pcy}{\hyperref[eqn:pcy]{\bm{\mathit{pcy}}}}
\newcommand{\suc}{\hyperref[eqn:suc]{\bm{\mathit{suc}}}}
\newcommand{\sym}{\hyperref[eqn:sym]{\bm{\mathit{sym}}}}
\newcommand{\aso}{\hyperref[eqn:aso]{\bm{\mathit{aso}}}}
\newcommand{\wf}{\hyperref[eqn:wf]{\bm{\mathit{wf}}}}
\newcommand{\tri}{\hyperref[eqn:tri]{\bm{\mathit{tri}}}}
\newcommand{\w}{\hyperref[eqn:w]{\bm{\mathit{w}}}}

\newcommand{\eqq}[1]{~\overset{\left(#1\right)}{=}~}
\newcommand{\eqqa}[1]{~\overset{\left(#1\right)}&{=}~}  % needs \usepackage{aligned-overset}
\newcommand{\eqqs}[1]{~\overset{\left(#1\right)}{\approx}~}

\newcommand{\ddx}[1]{\frac{\partial}{\partial#1}}

\newcommand{\linesep}{10pt}

% https://tex.stackexchange.com/questions/42726/align-but-show-one-equation-number-at-the-end
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\DeclareMathOperator{\doubled}{\text{doubled}}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "thesis"
%%% End:

